FileBounty: Fair Data Exchange

Digital contents are typically sold online through centralized and custodian marketplaces, which requires the trading partners to trust a central entity. We present FileBounty, a fair protocol which, assuming the cryptographic hash of the file of interest is known to the buyer, is trust-free and lets a buyer purchase data for a previously agreed monetary amount, while guaranteeing the integrity of the contents. To prevent misbehavior, FileBounty guarantees that any deviation from the expected participants' behavior results in a negative financial payoff; i.e. we show that honest behavior corresponds to a subgame perfect Nash equilibrium. Our novel deposit refunding scheme is resistant to extortion attacks under rational adversaries. If buyer and seller behave honestly, FileBounty's execution requires only three on-chain transactions, while the actual data is exchanged off-chain in an efficient and privacy-preserving manner. We moreover show how FileBounty enables a flexible peer-to-peer setting where multiple parties fairly sell a file to a buyer.

==> sections/1.Introduction.tex <==
\section{Introduction}
Fair multi-party exchange protocols have been extensively studied~\cite{kilincc2015optimally,garay2004efficient, gauthierdickey2014secure, bao1998efficient, asokan1998optimistic, dodis2003breaking, park2003constructing, zhou2000some, garay2003timed}. In light of the emergence of permissionless blockchains (e.g.\ Bitcoin), however, the design of fair exchange protocols has experienced a renaissance~\cite{banasik2016efficient,bentov2014use,bartoletti2016constant,andrychowicz2014fair, dziembowski2018fairswap}. The blockchain's properties allow to construct marketplaces without reliance on a centralized trusted third party (TTP), and instead enable the automated dispute mediation and integrated monetary transfers among buyers and sellers.

In this work, we first consider the following problem: we are given two participants, a seller and a buyer that are willing to exchange a digital file for a monetary amount. We assume that both parties mutually do not trust each other, and we therefore require a fair data exchange protocol. Our definition of fairness implies that a dishonest participant always suffers negative payoffs. In a second step, we consider the problem of a peer-to-peer (P2P) file exchange protocol similar to Bittorrent~\cite{cohen2008bittorrent}, whereby a buyer intents to purchase a file from multiple seller which are expect to be rewarded proportionally to their provided contents. We propose \name, a fair protocol that allows a buyer to purchase a digital file from a seller for a monetary amount. \name relies on the assumption that the buyer knows the cryptographic hash\footnote{Note in the extended P2P exchange protocol, we term the identity of a file \textit{fingerprint}.} of the file of interest (for example acquired through a semi-trusted third party, such as VirusTotal or a Torrent website\footnote{Note that we consider the semi-trusted third party offline, because it is not required to interact during or after the file exchange.}).

Given the file hash, a buyer e.g.~publishes on a blockchain an openly available bounty to purchase the file of interest from a willing seller. Alternatively, a seller can advertise its willingness to sell a file, similar to Bittorrent magnet links, connect with a buyer and complete the file and value transfer successfully. The file transfer is executed off-chain, i.e.\ the actual file content is not written on the blockchain; thus both protecting the privacy of the file and remaining scalable to any filesize. Even in the case of disputes, {\color{blue}no file content needs to be disclosed or, with a lower on-chain cost, at most one file block\footnote{e.g., $64$ bytes for files identified with SHA256, which amount to $0.0064$\% of a 1MB file} is released to the blockchain for each seller.} The file is moreover exchanged gradually and integrity protected, i.e.\ for each file chunk, which consists of multiple file blocks, transferred, the buyer can efficiently verify that a chunk is a valid chunk of the file of interest. We further extend \name to a distributed P2P setting, whereby a buyer can purchase the file of interest from multiple seller simultaneously, allowing the transfer speed to scale proportionally to the number of sellers and their network connectivity --- while minimizing the costs of a potential dispute process.

We adopt a rational adversarial model, under which, for each transferred chunk, the seller is guaranteed to receive a proportional payoff, as long as he doesn't become unresponsive (e.g.~times-out). The smart contract verifies the proper execution of the protocol to assure the correct participant payoffs and automatically handles dispute mediation. We introduce a deposit refunding scheme that guarantees that \name is secure against a rational adversary, i.e.\ the adversary will only follow the honest protocol which corresponds to the subgame-perfect Nash equilibrium. In other words, any deviation for any player (buyer, seller) from the honest protocol behavior will result in a financial loss to this player.
For our design, we make use of the chaining property of Merkle-Damg\aa rd-based hash functions (as in use in MD5~\cite{rivest1992md5}, SHA1~\cite{eastlake2001us}, SHA2~\cite{standard2002fips}, etc.)\footnote{Although SHA3~\cite{SHA3} is not relying on the Merkle-Damg\aa rd but on the Sponge construction, we believe that a similar design is feasible.}. %More specifically, we make use of the fact that given a file chunk of the input and the previous digest of the hash function, we can compute the following digest recursively. This enables the seller to gradually release the data while the buyer can verify that the data given is correct (i.e.\ corresponds to a file chunk of the file whose hash is known to the buyer).

Potential application opportunities of \name are extensive: 
(i) decentralized digital marketplaces,
(ii) purchase of sparsely seeded torrent files, (iii) decentralized file backups, 
(iv) brute-forcing of password hashes given their respective salts and 
(v) exchange of malware samples\footnote{i.e.\ \url{http://www.virustotal.com}}.

As a summary our contributions are as follows:
\begin{itemize}
	\item \textbf{Fair one-to-one Exchange} We propose \name{}, a fair data exchange protocol which allows a buyer (who knows the cryptographic hash of the file of interest), to make a publicly available bounty call for a digital file.
	\item \textbf{Fair Multi-Party Exchange} We present a novel multi-party exchange protocol based on BLS signatures, whereby a buyer can fairly purchase a file from multiple sellers.
	\item \textbf{Efficient Integrity Verification} By taking advantage of the Merkle-Damg\aa rd construction (e.g., in SHA256), our design allows the buyer (who only knows the file hash) to verify for each received file chunk, that the file chunk belongs to the file of interest.
	{\color{blue}
	\item \textbf{Privacy-Preserving} We conduct the on-chain dispute mediation in a privacy-preserving manner through zkSNARKs --- no content needs to be exposed to prove the possession.
	}
	\item \textbf{Nash Equilibrium} We show that \name is secure under a rational adversary, i.e.~we show that honest behavior is the subgame perfect Nash equilibrium. Misbehavior of any of the involved parties is detected while the data is gradually exchanged. Contrary to previous schemes, ours is resistant to extortion attacks under the rational adversary.
\end{itemize}

The remainder of the paper is organized as follows. In Section~\ref{sec:background} covers the background, Section~\ref{sec:design} presents the system and adversarial model and \name{}'s design. Section~\ref{sec:securityanalysis} focuses on the security analysis while we present our evaluation in Section~\ref{sec:evaluation}. We overview related work in Section~\ref{sec:relatedwork} and conclude the paper in Section~\ref{sec:conclusion}.

==> sections/2.Background.tex <==
\section{Background}\label{sec:background}
%In this section, we briefly discuss permissionless blockchains, game theoretic aspects, cryptographic hash functions and the Merkle-Damg\aa rd construction, required background knowledge for \name{}.
In this section, we briefly discuss permissionless blockchains, game theoretic aspects, etc., required background knowledge for \name{}.
\paragraph{\textbf{Blockchain}}
    In permissionless blockchains, any peer is free to join or leave at any moment the network. Proof-of-Work (PoW), introduced by ~\cite{dwork1992pricing}, is a computationally expensive puzzle that is the currently widest deployed mechanism to operate permissionless blockchains (e.g.\ Bitcoin). Besides the simple transfer of monetary value, transactions can execute a user-defined programs, commonly referred to as smart contracts, which alter the state of the blockchain. For an in-depth background, we refer the reader to~\cite{tschorsch2016bitcoin}.

    \paragraph{\textbf{Game Theory and Cryptoeconomics}} Fair multiparty protocols can be modeled as non-cooperative games, where each party acts rationally in its own best interest. The subgame perfect Nash equilibrium~\cite{osborne1994course} is a game theoretic solution concept of the extensive form game that we use in this paper to model the sequential interaction between the seller and the buyer. In this solution, each player plays the optimal strategy at each possible state. If any player would change its strategy in this solution, the expected financial gain is a non-positive number, as such, no player has an incentive to change its strategy in any state.
    
    %\paragraph{Cryptographic Hash Functions} The purpose of cryptographic hash functions is to map an arbitrary input sequence into a fixed-sized byte array --- similar to providing an identifier for a digital data file~\cite{goldwasser1996lecture,rivest1992md5,eastlake2001us,standard2002fips, SHA3}. Cryptographic Hash Functions should satisfy several properties, of which we detail the most relevant ones to this work. First, the same input sequence should always result in the same output hash. Second, it should be infeasible to generate a message from its hash (i.e.\ the hash should not reveal any information about the input to the hash function). Third, it should be infeasible to find so-called hash collisions. A hash collision occurs when two different input sequences are found, which result in the same hash value. The security of cryptographic hash functions is typically defined by how well they resist collision attacks, depending on which input sequence the adversary can choose from (any input corresponds to preimage resistance, a fixed input corresponds to second preimage resistance). Common cryptographic hash functions such as SHA1 and SHA256 make use of the Merkle-Damg\aa rd construction.
    
    \paragraph{\textbf{Merkle-Damg\aa rd and Sponge Construction}}
    The Merkle-Damg\aa rd construction~\cite{goldwasser1996lecture} allows to build a collision-resistant cryptographic hash function with an arbitrary size input from a collision-resistance one-way compression function. The arbitrary-length input data is divided into fixed-length data chunks and use an underlying cryptographic hash function in order to produce a final hash (cf. Figure~\ref{fig:merkledamgard}). For security purposes, the length of the actual input data needs to be appended at the end of the data. There are alternatives to the Merkle-Damg\aa rd construction, like for example the Sponge construction which is the basis for the SHA-3 hash function~\cite{SHA3}.
    
    \paragraph{\textbf{Boneh-Lynn-Shacham signature scheme}} The Boneh-Lynn-Shacham (BLS) signature scheme~\cite{boneh2001short} is a short digital signature technique using a bilinear pairing on a curve which supports signature aggregation~\cite{boneh2003aggregate} (e.g. compressing multiple signatures signed by different private keys on different messages in a single signature).

    {\color{blue}
    \paragraph{\textbf{Zero Knowledge Proofs}} In cryptography, zero-knowledge proofs (ZKP)~\cite{feige1988zero} allow a prover to prove to another verifier that a statement is true but without revealing any information of it. zkSNARKs~\cite{bitansky2012extractable} are succinct ZKP methods in which the size of the proof is small enough to be verified efficiently (e.g.~by a smart contract). zkSNARKs are moreover non-interactive i.e.\ no interaction is required between the prover and the verifier.
    }

\begin{figure}[!htb]
\centering
\includegraphics[width=0.3\textwidth]{figures/merkledamgard2.pdf}
\caption{Merkle-Damg\aa rd construction. The input file is divided into $m$ blocks, and the construction is initialized with a fixed initialization vector (IV). Intermediate states ($H_i$) represent temporary hashes, while the final file hash is output at the top. Note that the length of the file ($len$) is attached to the end of the file. Note that $H(F)$ corresponds to $H_m$.}
\label{fig:merkledamgard}
\end{figure}

==> sections/3.Overview.tex <==
\section{\name: Overview}\label{sec:design}
In this Section, we first outline the system and adversarial model followed by the detailed protocol specification.

\subsection{System Model}
In our system model, four parties are involved: (i) the seller, (ii) the buyer (iii) the semi-trusted third party which provides the cryptographic hash of the file of interest and (iv) the smart contract.
\begin{itemize}
    \item \textbf{Permissionless Blockchain} We assume the existence of a permissionless (e.g.\ Proof-of-Work) blockchain that supports the convenient deployment of smart contracts. Participants have identities in the form of public keys that are tied to their respective private keys ($Pub_x/Priv_x$) to perform e.g.\ digital signatures.
    \item \textbf{Buyer} The buyer $B$ is the entity which is willing to purchase the file $F$ with cryptographic hash $H(F)$ from a seller for a given price $F_p$. 
    \item \textbf{Seller} The seller $S$ is the entity which claims to own and is willing to transfer the digital file $F$, corresponding to the cryptographic hash $H(F)$, to a buyer.
    \item \textbf{Semi-trusted third party} The semi-trusted third party plays (STTP) the role of coordinator, which provides the cryptographic hashes of files to buyers, keeps track of seller's availability at the time of requests and assists peers in communication establishment.
    
    \end{itemize}

    To exchange the file $F$, we assume a communication protocol external to the blockchain, which requires the buyer or the seller to directly connect (e.g.\ over WebRTC). %provide a publicly reachable IP address as well as an open TCP or UDP port. The other participant then connects to this port and the execution of the protocol begins.
    
    \begin{itemize}
    \item \textbf{Iterated Hash Functions} Our protocol relies on iterated hash functions~\cite{lucks2004design} (such as SHA256). An iterated hash function takes a message $M \in \{0,1\}^{*}$ of any length to compute an s-bit output H(M). For an iterated hash, we split the padded message into $m$ fixed-sized parts $M_1, M_2, ..., M_m \in \{0, 1\}^{l}$. An iterated hash $H$ iterates an underlying compression function $f$, and the final hash is given by $f(f(... f(f(H_0, M_1), M_2) ...), M_m)$, where $H_0$ is some constant initial value usually denoted as Initialization Vector ($IV$).
\end{itemize}
We term the fixed-sized parts of a file fed into the integrated hash functions \textit{blocks} in this paper. Adjacent file blocks are bundled to \textit{chunks} as the transmission unit. In the P2P scheme, files are split into \textit{segments} which are exchanged separately. Segments are exclusive parts of a file containing several file chunks. Figure~\ref{fig:merkledamgard} illustrates the relationship between the three terms.

% \begin{description}
% {\color{blue}
%     \item[File Block] 
%     \item[File Chunk] 
%     The file $F$ is divided into $m$ blocks with a fixed block size(BLOCK\_SIZE) which depends on the chosen cryptographic hash function (e.g. 64 bytes for SHA-256). The file will be transmitted in $n$ chunks. Each chunk consists of a fixed number(CHUNK\_LEN) of blocks (cf\. Equation~\ref{eq:filechunk}), s.t.\ $n=\lceil m/\text{CHUNK\_LEN} \rceil$.
%         \begin{equation}\label{eq:filechunk}
%         \begin{split}
%           c_k = \left\{
%             \begin{array}{@{}l@{\thinspace}l}
%               M_1\ ||\ ...\ ||\ M_{m-(n-k)CL} &\text{,if } k=1 \\
%               M_{m-(n-k+1)CL+1}\ ||\ ...\ ||\ M_{m-(n-k)CL} &\text{,otherwise} \\
%             \end{array}
%           \right.\\
%           CL=\text{CHUNK\_LEN},\ ||\text{ represents concatenation}
%         \end{split}
%         \end{equation}

%     Note the length of $c_1$ is not necessarily equal to CHUNK\_LEN. The intermediate hash of $c_k$ is same as the intermediate hash of its last block (i.e. $H_k^c = H_{m-(n-k)CL}$). For the convenience of the reader but without loss of generality, we assume each chunk contains one block (i.e.\ $\text{CHUNK\_LEN} = 1$) in the rest of this paper.

%     \item[File Segment] files are split into segments, which are exchanged separately. Segments are exclusive parts of the file which are composed of adjacent file chunks. Contrary to one-to-one scheme where each file is identified by a hash value, multi-to-one transfer requires the bundle of all the segments' hashes as the identity so that the authenticity of every segment can be verified individually. Similar to the chunk hash, the segment hash is also defined as the intermediate hash of the last block inside the segment, which means there is no additional computing overhead for segment hashes.
%     }    
% \end{description}


\subsection{High-Level Operation}

We outline the high-level operations of \name{} in Figure~\ref{fig:overview}, which is divided into four phases.
%The \name{} protocol can be divided into four phrases. \todo{needs to account for the case of multiple sellers}
\begin{itemize}
    \item \textbf{Setup Phase} %{In the setup phase, the seller and the buyer agree on the necessary parameters and submit the information to the smart contract along with the deposits.}
    In the setup phase (a), the sellers start to serve a file $F$ by submitting a set of requisite parameters and the deposit $D_S$ to the smart contract. The buyer who is interested in $F$ can pay the file price $F_P$ with the deposit $D_B$ and initiate off-chain communication channels to the alive sellers.
    \item \textbf{File Transfer Phase} %{The seller transfers the file to the buyer in chunks. The transmission is performed in the pre-established communication channel, which is considered to be secure. The buyer needs to send back a signature as the acknowledgement every time receiving a chunk. }
    Once the on-chain transactions confirmed in the setup phase and the off-chain channels are established, the protocol enters into the file exchange phase (b). The buyer receives $F$ in chunks from one or multiple sellers. For each transferred chunk, the client verifies the chunk's integrity given the file hash $H(F)$ and the seller receives a signed acknowledgment from the buyer.
    \item \textbf{Dispute Phase} {Either side can report to the smart contract if the opposite misbehaves (c). The opposite then is able to respond within the given time. If both sides behave honestly till the end of transmission, the protocol will go to the payoff phase directly.}
    \item \textbf{Payoff Phase} {In the payoff phase (d), the smart contract allocates the file price and the deposits to the buyer and the seller according to the execution of the protocol.}
\end{itemize}

\begin{figure*}[!htb]
\centering
\includegraphics[width=0.5\textwidth]{figures/overview.pdf}
\caption{Four phases of  \name{} --- (a) setup phase; (b) file exchange phase; (c) dispute phase; (d) payoff phase.}
\label{fig:overview}
\end{figure*}

\subsection{Main Properties}
\begin{itemize}
    \item \textbf{Permissionless Blockchain} Blockchain transactions enable a certain transaction throughput and bear a cost borne by the buyer and seller.
    \item \textbf{Buyer} The buyer is able to establish a secure communication channel to the seller and interacts with a blockchain-based smart contract. Prior to the exchange, the buyer provides a monetary deposit of value $D_B$. The file of interest is worth $F_v$ to the buyer.
    \item \textbf{Seller} The seller is able to establish a secure communication channel to the buyer and interacts with the blockchain-based smart contract. Prior to the file exchange, the seller provides a monetary deposit of value $D_S$. The seller's costs for selling the file amounts to $F_c$.
    \item \textbf{Semi-trusted third party} The STTP only assists in the trade and is not involved in the exchange of any monetary nor data transfer between the buyer and the seller.
    % \todo{please rewrite}{\color{orange}We denote this third party as semi-trusted because assuming the third party is not colluding with the seller, the third party is not involved in the exchange of any monetary nor data transfer between the buyer and the seller. The buyer could moreover rely on multiple semi-trusted third parties which could confirm the same cryptographic hash for the file of interest.}
\end{itemize}

\subsection{Attacker Models}
\label{sec:attackermodels}
We assume that the underlying blockchain is reasonably resistant against 51\% and double-spending attacks. We moreover assume that the consensus mechanism of the blockchain achieves eventual consistency and that the transactions are non-repudiable and non-malleable. We also assume, that \name{}'s smart contract implementation is secure~\cite{luu2016making}. Additionally, we rely on the correct design and implementation of the cryptographic primitives of the blockchain.

We consider off-chain connection between the seller and buyer secure and stable that can't be controlled by any adversary. All protocol participants are assumed to be able to monitor the state changes of the smart contract and respond timely.

We assume the STTP is not colluding with the seller. We also assume a rational adversary, i.e.\ an adversary that is motivated by financial gain. As such, our adversary is not interested in provoking the opponent to lose a monetary amount during the protocol execution as it would entail a loss for the adversary as well.

\begin{itemize}
    \item \textbf{Malicious Seller} A malicious seller might stop sending file chunks during transmission that the incomplete file the buyer receives is worthless (e.g. compressed file). A malicious seller may also dishonestly report the buyer (e.g.\ pretending not to receive the acknowledgement from the buyer) causing the possibility that the smart contract affirm misbehaviour of the buyer, or try to blackmail the buyer during the execution of the protocol otherwise the buyer might lose more economically. We analyze the irrationality of extortion attacks in Section~\ref{attack_analysis}. In the P2P exchange different sellers can collude with each other (e.g. interrupting one exchange thread, the buyer then can't receive the complete file).
    \item \textbf{Malicious Buyer} As \name{} is sequential, a malicious buyer may operate similar attacks (i.e.\ refusing to acknowledge a file chunk so that the seller can't prove the delivery of a chunk, reporting dishonestly and extortion attacks).
\end{itemize}

% As our protocol relies on timeouts, and a permissionless blockchain acts as a timestamping service, we can choose to either use the block height or the block timestamp (UNIX timestamps). The Ethereum blockchain enables smart contract to track time by using $block.timestamp$. Miners do not accept blocks whose timestamp is more than 900 seconds after the previous one~\cite{blockvalidationalgorithm}. Because $MAX\_TIMEOUT$ is chosen to be significantly larger than the block time of Ethereum, it is economically not feasible to alter the time-stamping mechanism.

% We assume that the buyer $B$ and the seller $S$ are capable of communicating over a non-blockchain based channel. This channel is not required to be secure and will solely be used for the purpose of negotiating the terms of the contract.

% Note that \name{}, in its original form, does not support the resumption of a previously failed protocol execution. We leave the extension for future work.

% Note that as transactions on the blockchain have a cost, it must hold that the total transaction costs are much lower than the value put into the smart contract, i.e.\ $F_p + D_B + D_S$  (cf. Section~\ref{sec:evaluation}).

% \clearpage

==> sections/4.Details.tex <==
\section{\name~Details}
In the following we outline \name's details.

\subsection{Formal Overview}
We first depict \name in detail for the single seller case. We consider the buyer $B$ is willing to purchase the file $F$ with the hash $H(F)$ from the seller $S$ who claims to possess it.

We present in Algorithm~\ref{alg:protocol_pseudocode} the pseudocode of the \name{} protocol which the seller and the buyer iteratively execute for each chunk.

\name{} supports the following events:
\begin{itemize}
    \item $T_k$ corresponds to $S$ transmitting the file chunk~$c_k$.
    \item $A_k$ is the acknowledgment of file chunk $c_k$ by $B$.
    \item If one participant does not follow the honest behavior, then the other party ($x$) can report to the smart contract for chunk $c_k$ which we denote $R^x_k$.
    \item $P_k^x$ signifies that one party (x) proves to the smart contract for chunk $c_k$ to resolve a dispute, e.g., $B$ publishes a block on the blockchain.
    \item Not proving a chunk $\overline{P_k^x}$ equals to being offline ($\bot^x$).
\end{itemize}
Notations adopted in this paper are given in Table \ref{tb:notation}.

\begin{algorithm}[htb]\label{alg:protocol_pseudocode}
 \KwData{$Pub_B, Pub_S, F_p, D_B, D_S, ...$}
 \KwResult{Buyer gets file F, seller is paid $F_p$}
 initialization: set up of a secure channel\;
 \For{$k = n..1$}{
  \textit{Seller sends current chunk $c_k$ and intermediate hash $H_{k-1}^c$\;
  Buyer verifies that $f(f(...f(H_{k-1}^c,M_{CL}^k)...),M_1^k) = H_k^c$\;}
  \eIf{Integrity check is okay}{
   \textit{Buyer signs acknowledgement $A_k$ and sends it to Seller\;
   Seller verifies the validity of the signed acknowledgement\;}
    \If{$A_k$ is NOT valid}{
     \textit{Seller reports to the smart contract that the buyer misbehaved\;}
    }
   }{
   \textit{Buyer reports to the smart contract that the seller misbehaved\;}
  }
 }
\textit{ Seller finanlizes the exchange to withdraw deposits of both participants;} 
% $confirmChunk(A_1)$ to finalize the protocol\;
%  Both participants separately call
%  withdraw() to get their deposit back\;}
 \caption{Outline of \name{}'s transfer protocol. Dispute mediation is discussed in Section~\ref{disputemediation} and the details are given in Table~\ref{tab:payouts}.}
\end{algorithm}

\begin{table}[!htb]\centering\small
\caption{Notations adopted for this work.}\label{tb:notation}
\begin{tabular}{ll}
\toprule
Notation & Description \\
\midrule
$F $     & File to be sold\\
$M_i$    & File block $i$\\
$H_i$    & Intermediate hash of $M_i$\\
$h(M)$   & Intermediate hash of block $M$\\
$c_k$    & File chunk $k$\\
$H_k^c$  & Intermediate hash of $c_k$\\
$M_i^c$  & The $i_{th}$ block in $c_k$\\
$s_q$    & File segment $ q$\\
$H_q^s$  & Intermediate hash of $s_q$\\  
$S$      & Seller of the file $F$\\
$B$      & Buyer of the file $F$ \\
$D_S$    & Deposit of the seller \\
$D_B$    & Deposit of the buyer\\
$F_v$    & File value for the buyer\\
$F_p$    & File price paid by the buyer\\
$F_c$    & File selling costs for the seller\\
$T_k$    & Seller successfully transmitted file chunk $k$\\
$A_k$    & Buyer signed ack. of file chunk $k$\\
$R^x_k$  & $x$ reports the other party faulty at chunk $k$\\
$P_k^x$  & $x$ proves to settle a dispute\\
$\bot^x$ & Party $x$ is considered offline\\
$g^x(k)$ & Rel. utility for $x$ after $k$ transferred chunks\\
\bottomrule
\end{tabular}
\end{table}

%For a schematic overview of \name{}, we refer the reader to Figure~\ref{fig:overview}. We consider the buyer $B$ to be the initiator of the protocol, communicating with the seller and file owner $S$ over some (not necessarily secure) channel. $B$ is willing to purchase the file $F$ from $S$ who claims to posses the file with the hash $H(F)$. In order to proceed, $B$ and $S$ agree in the initial setup phase on the following set of parameters.

\subsubsection{\textbf{Setup Phase}}
{\color{blue}In the setup phase, $B$ should accept the initial parameters set by $S$ in order to proceed. $B$ and $S$ should agree on the monetary file price $F_p$ and their respective deposits accordingly (cf.\ Section~\ref{sec:nashequilibrium}), which are required in case of dispute mediation. We assume that $B$ and $S$ have their respective public keys $Pub_B$ and $Pub_S$, which correspond to their respective blockchain addresses.
%The first parameter that $B$ and $S$ agree on is the monetary file price $F_p$. Based on the file price, they decide on their respective deposits (cf. Section~\ref{sec:nashequilibrium}), which are required in the case of dispute mediation. We assume that $B$ and $S$ have their respective public keys $Pub_B$ and $Pub_S$, which correspond to their respective blockchain addresses.

The file $F$ is divided into $m$ fixed-size ($BLOCK\_SIZE$) blocks for the hash calculation. $BLOCK\_SIZE$ is determined by the chosen cryptographic hash function (e.g. 64 bytes for SHA-256).

The file will be transmitted in $n$ chunks. Each chunk consists of a fixed number ($CHUNK\_LEN$ abbr. $CL$) of blocks (cf. Equation \ref{eq:filechunk}), s.t.\ $n=\lceil m/CL \rceil$.
%The block size (BLOCK\_SIZE) is determined by the chosen cryptographic hash function (e.g. 64 bytes for SHA-256). The file $F$ is divided into $m$ blocks with a fixed block size(BLOCK\_SIZE) which depends on the chosen cryptographic hash function (e.g. 64 bytes for SHA-256). The file will be transmitted in $n$ chunks. Each chunk consists of a fixed number(CHUNK\_LEN) of blocks (cf\. Equation~\ref{eq:filechunk}), s.t.\ $n=\lceil m/\text{CHUNK\_LEN} \rceil$.
\begin{equation}\label{eq:filechunk}
\begin{split}
  &c_k = \left\{
    \begin{array}{@{}l@{\thinspace}l}
       M_1\ ||\ ...\ ||\ M_{m-(n-k)CL} &\text{,if } k=1 \\
       M_{m-(n-k+1)CL+1}\ ||\ ...\ ||\ M_{m-(n-k)CL} &\text{,otherwise} \\
    \end{array}
   \right.\\
  %&||\text{ represents concatenation}
\end{split}
\end{equation}

Note the length of $c_1$ is not necessarily equal to $CL$. For the convenience of the reader but without loss of generality, we assume $c_1$ contains $CL$ blocks in the rest of this paper.  We denote the $i_{th}$ block of chunk $c_k$ as $M_i^k$ and its intermediate hash as  $h(M_i^k)$. The intermediate hash of $c_k$ is same as the hash of its last block, i.e.\ $H_k^c = h(M_{CL}^k)$.

To make sure that the protocol terminates, we define as $MAX\_TIMEOUT$ the maximum time that a participant has to respond before being considered offline. As a permissionless blockchain acts as a timestamping service, we can choose to either use the block height or the block timestamp (UNIX timestamps). The Ethereum blockchain enables smart contract to track time by using $block.timestamp$. Miners do not accept blocks whose timestamp is more than 900 seconds after the previous one~\cite{blockvalidationalgorithm}. Because $MAX\_TIMEOUT$ is chosen to be significantly larger than the block time of Ethereum, it is economically not feasible to alter the time-stamping mechanism.

Summarily, in the setup phase $B$ and $S$ should agree on the file price $F_p$, deposits $D_B$, $D_S$, $BLOCK\_SIZE$, $CHUNK\_LEN$ and $MAX\_TIMEOUT$ and deposit to the smart contract respectively to kick off the transmission.}
%Given these initial parameters, $B$ compiles and deploys the \name{} smart contract to a publicly available blockchain with the file price $F_p$ and the deposit $D_B$. $B$ transmits the source code of the contract to $S$, so that the seller can compile and verify that the smart contract deployed on the blockchain indeed corresponds to the \name{} contract. $S$ then sends the deposit $D_B$ to the smart contract.%\footnote{\name{} is also suitable for the scenario that the seller initiate the protocol. For example, the seller can serve the file by setting the parameters in advance and deposit $D_S$ to the smart contract. If there is no disagreement, the buyer can then try to connect to the seller and pay $F_p + D_B$ to start the transmission.}

\subsubsection{\textbf{File Transfer Phase}}
We assume that $S$ and $B$ are now capable of connecting off-chain. $S$ starts by sending $B$ the chunk $c_n$ and the intermediate hash $H_{n-1}^c$ (cf. Figure~\ref{fig:merkledamgard}).%, we denote this action by $S_n$.

After having received $c_n$, the buyer verifies that $f(f(...f(H_{n-1}^c,M_{CL}^n)...),M_1^n) = H(F)$. Note that $f(\cdot)$ corresponds to the one-way compression function, while $H(\cdot)$ corresponds to the iterated compression function over the whole input. % (e.g.\ Merkle-Damg\aa rd).
If the hash is correct, $B$ signs an acknowledgment, $A_n$, and sends it to $S$. The acknowledgment states, that the valid file chunk $c_n$ was received by the buyer. %Thus, in case of disputes, the seller is able to broadcast the buyer's acknowledgment $A_n$, confirming that the seller properly transmitted the respective file chunk.
$S$ then continues the protocol by giving $B$ the next file chunk $c_{n-1}$ and the intermediate hash $H_{n-2}^c$, to which $B$ answers by signing the acknowledgment $A_{n-1}$.

For every $k \in \{1,2,...,n\}$, $S$ sends $B$ the file chunk $c_{k}$ and the intermediate hash $H_{k-1}^c$, to which $B$ responds by signing $A_{k}$. By the definition of the Merkle-Damg\aa rd construction, $H^c_0 = H_0 = IV$, the initialization vector.
\subsubsection{\textbf{Dispute Phase}}
\label{disputemediation}
{\color{blue}Either player is able to report the misbehaviour of the adversary in the transmission. Note that we consider non-responsiveness to be malicious. Both the buyer and the seller are therefore incentivized to respond during the execution of the protocol (within $MAX\_TIMEOUT$). In the following paragraphs, we discuss how to handle the misbehavior of either the seller or the buyer.

\paragraph{\textbf{Misbehavior of the seller}}
If $S$ interrupts the protocol or sends an incorrect file chunk at any point during the file transfer phase, $B$ can notify the smart contract that $S$ behaved incorrectly, noted $R^B_k$. $S$ then has $MAX\_TIMEOUT$ to prove the possession of the last block of $c_k$ (i.e.\ $M_{CL}^k$). \name offers two proof methods --- 1.~$S$ publishes $M_{CL}^k$ and the digest (i.e.\ $h(M_{CL-1}^k)$) directly to the smart contract; then, the smart contract verifies that $f(h(M_{CL-1}^k),M_{CL}^k) = H_k^c$. 2.~$S$ sends the zkSNARKs proofs to the smart contract without revealing any content of $F$, which is more privacy-preserving but consumes a higher on-chain cost. $S$ can choose the appropriate solution according to the value of $M_{CL}^k$. Depending on whether $S$ provides a valid proof, the smart contract assigns different payoffs to $S$ and $B$. We refer the reader to Section~\ref{payoffphase} for the exact payoff calculation.

\paragraph{\textbf{Misbehavior of the buyer}}
{\color{blue}  $S$ can report $B$ at any moment if the buyer acknowledges a chunk $c_k$ without having received it\footnote{This may look counter-intuitive, but this functionality enables us to remove the possibility of extortion attacks from the rational seller, as explained in section \ref{sec:nashequilibrium}}, noted $R^S_k$. The smart contract then allows $B$ within $MAX\_TIMEOUT$ to prove the knowledge of $h(M_{CL-1}^k)$ and $M_{CL}^k$, s.t. $f(h(M_{CL-1}^k),M_{CL}^k) = H_k^c$ (similar to the case of seller's misbehavior). $S$ can also report $B$ for not responding an acknowledgement $A_k$ by submitting the last received acknowledgement $A_{k+1}$.}

% {\color{red}
% The seller can report the buyer, noted $R^S_k$, at any moment if the buyer acknowledges a chunk without having received it\footnote{This may look counter-intuitive, but this functionality enables us to remove the possibility of extortion attacks from the rational seller, as explained in section \ref{sec:nashequilibrium}}. The smart contract then allows the buyer during $MAX\_TIMEOUT$ to provide the current chunk data that is being disputed to the smart contract (similar to the case of seller misbehavior).
% }
\subsubsection{\textbf{Payoff Phase}}
\label{payoffphase}
Supposing that both parities behave honestly, once $S$ receives the acknowledgment of $A_1$ from $B$, $S$ can submit it to the smart contract to terminate the protocol. In this case, $S$ receives both the file price $F_p$ and the deposit $D_S$, while $B$ receives the deposit $D_B$ and has received the file $F$ through the off-chain communication channel. %In the case of a dispute, we refer the reader to Section~\ref{sec:payofffunction} for the fair payoff amounts depending on the protocol execution.

Depending on the protocol execution steps, for example in case of disputes, we define the particular payouts for the seller and the buyer. We distinguish between the payout defined by the smart contract (i.e., the monetary amount that the smart contract pays) and the utility function (i.e., the utility of the seller and buyer for each chunk of the file).

We summarize the corresponding payouts for each protocol step in Table~\ref{tab:payouts}. For the ease of understanding, we provide a visual representation in Figure~\ref{fig:payouts}.

}

\begin{figure*}[!htb]
\centering
\includegraphics[width=0.7\textwidth]{figures/tree_start.pdf}
\caption{Payoff values for the seller and the buyer, depending on the protocol transition steps for two file chunks. $S$ stands for the seller, $B$ stands for the buyer. For each payoff, we distinguish between the payoff by the smart contract (left side) and the utility payoff (right side). For each payoff, the upper payoff concerns the buyer, while the lower concerns the seller. If one participant does not follow the protocol (i.e does not send a chunk, does not acknowledge or goes offline), then the other ($x$) can initiate a dispute for chunk $k$, denoted $R^x_k$; it is then up to the first participant to resolve the dispute. To simplify the presentation, we omitted some sub-cases where a participant becomes offline and also the branch in which buyer acknowledges the receipt of the file chunk in case of not receiving it; for details, please refer to Table~\ref{tab:payouts}.} \label{fig:payouts}
\end{figure*}


% We further exemplify how the dispute mediation system operates. For simplicity, we assume a file made of 4 chunks. We further assume that the seller possesses the file, as otherwise the seller's deposit would be burned and the buyer would be refunded.

% \subsubsection{Seller sends no chunk}
% Both the buyer and the seller provided their deposit to the smart contract, yet the seller refrains from sending the first chunk $c_n$ = $c_4$ to the buyer. The buyer can then report the non-reception of file chunk $k$ that we denote by $R^B_k$. This notifies the smart contract that the sender didn't send the chunk $k$. The seller then has $MAX\_TIMEOUT$ time to send $c_4$ and the intermediate hash $H_3$ to the smart contract such that $f(c_4, H_3) = F(H)$; if this condition is fulfilled, the smart contract sets the payoffs as follows:
% \begin{align}\label{Eq:1}
%  \text{Buyer:~} & \dfrac{3}{4} \cdot F_p &
%  \text{Seller:~}& \dfrac{1}{4} \cdot F_p
% \end{align}


% Otherwise, if the seller times out or does not provide a correct pair ($c_4$, $H_3$), then the payoffs are the following:
% \begin{align}\label{Eq:2}
%  \text{Buyer:~} & F_p + D_B &
%  \text{Seller:~}& 0
% \end{align}

% Note that the seller's deposit is burned (i.e.\ destroyed) and not refunded.

% \subsubsection{Seller sends the chunk but buyer reports him anyway}
% From the point of view of the smart contract, this case is equivalent to the previous one. The reason is that the smart contract has no means of verifying whether the seller sent the chunk to the buyer. Consequently, the payoffs are the same.

% %\subsubsection{Seller sends only first chunk}

% \subsubsection{Seller sends all but the last chunk}
% The protocol has been correctly executed until the last chunk, which for some reason the seller does not send. 
% If the buyer acknowledges the receipt of the file chunk although he did not receive it, then the seller reports the wrong acknowledgment of the chunk receipt $R_{1}^S$ and the buyer is unable to prove the receipt of the chunk. Therefore, the seller gets all the deposits from the smart contract, namely $D_S+D_B+F_p$, while the buyer gets $0$. This implies that the buyer will not acknowledge the receipt of the chunk if he actually does not receive it.

% Consequently, the buyer claims the non-reception of file chunk $c_1$ by reporting. 

% The seller then has $MAX\_TIMEOUT$ time to send $c_1$ and the intermediate hash $H_0 = IV$ to the smart contract such that $f(c_1, H_0) = H_1$; if this condition is fulfilled, the smart contract sets the payoffs as follows:
% %\begin{align}%\label{Eq:3}
% %\begin{array}
% % &\text{Buyer:} ~ 0 \\
% % &\text{Seller:}~F_p
% %
% %\end{align}
% \begin{align}\label{Eq:4}
%  \text{Buyer:~} & 0 &
%  \text{Seller:~}& F_p
% \end{align}

% Note that both deposits are burned in this case.

% If the seller times out or does not provide a correct pair ($c_1$, $H_0$), then the payoffs are the following:

% \begin{align}\label{Eq:5}
%  \text{Buyer:~} &  F_p + D_B &
%  \text{Seller:~}& 0
% \end{align}

% \subsubsection{Buyer does not acknowledge the first chunk}
% Both participants have deposited money into the smart contract and started the execution of the protocol. The seller sends the first chunk $c_4$, yet the buyer does not acknowledge the reception of the first chunk. The seller therefore reports the buyer for allegedly timing out (by calling the report() function). The buyer then has $MAX\_TIMEOUT$ to confirm the termination of the protocol.

% Termination of the protocol:
% \begin{align}\label{Eq:6}
%  \text{Buyer:~} &  F_p &
%  \text{Seller:~}& 0
% \end{align}

% Buyer times out: 
% \begin{align}\label{Eq:7}
%  \text{Buyer:~} &  0 &
%  \text{Seller:~}& \dfrac{1}{4} \cdot F_p + D_S
% \end{align}
% % \kaihua{"The buyer, after initiating the protocol, blackmails the seller into sending X, or else the buyer will simply stay quiet. Note that in this case, if the seller reports, the buyer can terminate the protocol, which results in the seller losing his deposit; if the seller doesn't report he also loses his deposit."

% % Here, seemingly, we can't resist such an attack. What's the reason of refunding $D_B$ to Buyer?
% % }
% \subsubsection{Buyer does not acknowledge last chunk}
% Both participants have executed the protocol almost up to the end, the seller sent the last chunk $4$ but for some reason the buyer did not acknowledge the reception of this last chunk. Similarly to previous case, the seller reports the buyer for allegedly timing out. The buyer then has $MAX\_TIMEOUT$ to confirm that he is online, in which case it is up to the seller to prove to the smart contract that he sent the last chunk. If the buyer times out:
% \begin{align}\label{Eq:8}
%  \text{Buyer:~} &  0 &
%  \text{Seller:~}& F_p + D_S
% \end{align}

% The buyer confirms to be online\footnote{By calling the $setLastAppearance()$ function in the smart contract, which sets the lastAppearanceOfSeller respectively lastAppearanceOfBuyer to the actual timestamp. It is then up to the next participant to answer within the given timeframe, otherwise the first one will be able to end the protocol and considers the other participant offline.} by notifying the smart contract, we remain with two cases. First, the seller proves he sent the chunk:
% \begin{align}\label{Eq:9}
%  \text{Buyer:~} &  0 &
%  \text{Seller:~}& F_p
% \end{align}

% Second, the seller does not prove he sent the chunk (either is offline or does not provide a correct proof to the smart contract):
% \begin{align}\label{Eq:10}
%  \text{Buyer:~} &  \dfrac{1}{4} \cdot F_p + D_B &
%  \text{Seller:~}& 0
% \end{align}

% The last two cases are formally treated in the Table~\ref{tab:payoutsdetails}.

% Given these payoff examples, we now explain the security analysis of \name{}.

{\color{blue}
\subsection{Extension to a Multi-Party File Exchange}
In the P2P exchange setup, files are split into $z$ segments (e.g. a 1MB file can be divided into eight 128KB file segments). 
We extended the fingerprint of a file to the list of all segments' hashes (i.e.\ $\{H_1^s||H_2^s||...||H_z^s\}$). Similar to file chunks, we take the intermediate hash of the last block in segment $s_q$ as the segment hash $H_q^s$. $H_q^s$ is used as the target hash for $s_q$ in the exchange, as well as the initial vector for $s_{q+1}$, so that the buyer can verify the integrity of each segment. We can easily find $H_z^s=H(F)$. In the P2P setup, the smart contract needs to store additional parameters, namely the hash list and the segment size. Based on these, segments can be exchanged separately and concurrently --- segments are transmitted in chunks; the dispute mediation and the payoffs of all segments are independent.

We consider the buyer $B$ is willing to purchase a $z$-segment file $F$ with fingerprint $\{H_1^s||H_2^s||...||H_z^s\}$ from $z$ sellers $S_1, S_2, ..., S_z$. We assume all seller are sharing $F$ at the same price (i.e.\ $F_p/z$ per segment) and deposit (i.e.\ $D_S/z$ per segment). The P2P extension is executed as follows. 
\begin{itemize}
    \item \textbf{Serving} {Each seller starts to share $F$ by sending a transaction with the required parameters (i.e. the fingerprint etc.) and enough deposits which at least exceeds $D_S/z$. The amount of deposits determines the number of segments that can be exchanged concurrently.}
    \item \textbf{Handshake} {$B$ is required to prove the willingness of selling a specific chunk of each seller before initiating the exchanges. $B$ thus requests segment $s_q$ from seller $S_q$ with an off-chain message (cf. Equation~\ref{equ:requestmessage}).
    \begin{equation}\label{equ:requestmessage}
        \begin{split}
            r_{s_q} = \{\ &\mbox{id}:id,\ \mbox{valid\_period}:valid\_period\\
              &\mbox{buyer}:Pub_B,\  \mbox{seller}:Pub_{S_q},\\
              &\mbox{fingerprint}:H_1^s||H_2^s||...||H_z^s,\\ &\mbox{segment}:H_q^s\ \}
        \end{split}
    \end{equation}
    %$id$ is a random number which identifies the exchange thread and shared among all the $z$ exchange threads. A valid period is included to protect an offline seller from being attacked by a malicious buyer with a 
    The seller $S_q$ then signs the valid request as the confirmation. We utilize the BLS signature scheme which allows $B$ to aggregate $z$ signatures into a short one so that the smart contract can validate it efficiently. Once all the confirmations received, $B$ then sends the combination of the requests with the aggregated signature, the total price and the deposits to the smart contract.}
% \begin{figure}[!htb]
% \centering
% \includegraphics[width=0.3\textwidth]{figures/BLS.pdf}
% \caption{}
% \label{fig:BLS}
% \end{figure}
    \item \textbf{Transfer} {All sellers send chunks to $B$ in descending order. $B$ verifies the authenticity of every received chunk.
    \item \textbf{Dispute} The exchange threads are considered to be separate which means that any dispute is mediated independently. The dispute payoff scheme of the P2P scheme imitates the one-to-one exchange.}
    \item \textbf{Payoff} {After receiving all the segments, $B$ can notify the smart contract to redeem the deposits with an on-chain transaction. The file price will be sent to the seller directly and the sellers' deposits are unlocked in the smart contract for recycling.}
\end{itemize}

The recycling mechanism facilitates the repeatable selling with one on-chain transaction, which reduces the margin cost of sellers. For a P2P trade, only two on-chain transactions are required (i.e. 1.~the buyer initiates the transaction; 2.~finalizing the transaction).

Note that the same file can be priced differently by distinct sellers and we leave such specification for further work.
}

==> sections/5.Security.tex <==
\section{Security Analysis}\label{sec:securityanalysis}
In the following section, we outline the security analysis of \name. We first focus on the single seller case\footnote{We extend this to a cryptographic analysis in Appendix~\ref{apx:cryptographicanalysis}} and extend to the multi-party case in Section~\ref{sec:securemultipartyexchange}.


% In this section, we outline the security analysis of \name{}\footnote{We extend this to a cryptographic analysis in Appendix~\ref{apx:cryptographicanalysis}} with a focus on the single seller case. We regard the P2P exchange as multiple independent threads of single seller exchanges, each thread holds the same security properties. We prove in Appendix~\ref{proof} that honest behavior corresponds to a subgame perfect Nash equilibrium in a single thread, which implies that following the protocol in all threads is the optimal behavior for colluding sellers.
% In the following section, we detail the security analysis of \name{} by first outlining the security assumptions and subsequently proving that honest behavior in \name{} is a Nash equilibrium.

% \subsection{Adversarial Model and Assumptions}
% We assume a rational adversary, i.e.\ an adversary that is motivated by financial gain. As such, our adversary is not interested in provoking the opponent to lose a monetary amount during the protocol execution as it would entail a loss for the adversary as well.
% \begin{description}
% \item[Fairness definition]
% Similar to Franklin et al.~\cite{franklin1997fair}, we consider a protocol fair if the file exchanged is consistent with the known hash value and the monetary amount is transferred. We moreover require, that a seller without knowledge of the file cannot cause any economical damage to the other party. To summarize, we consider a file exchange protocol fair, if an honest participant of the protocol cannot be forced to lose monetary value, under a rational adversary
% %
% \item[Security Assumptions]
% We assume that the underlying blockchain, i.e.\ the underlying consensus protocol, is secure. We rely on a permissionless blockchain (e.g., Ethereum), meaning that both buyer and seller can generate a valid public/private key-pair ($Pub_S/Priv_S$ and $Pub_B/Priv_B$, respectively) and corresponding addresses to create transactions. The currently most prevalent consensus protocol for permissionless blockchains is Proof of Work. We assume, that the blockchain is reasonably resistant against double-spending and selfish mining attacks~\cite{gervais2016security}. We moreover assume that the consensus mechanism of the blockchain achieves eventual consistency (a property of Proof of Work), and that the transactions are non-repudiable and non-malleable (satisfied by Ethereum). We also assume, that \name{}'s smart contract implementation is secure~\cite{luu2016making}. Additionally, we rely on the correct design and implementation of the cryptographic primitives of the blockchain.
% \end{description}
% As our protocol relies on timeouts, and a permissionless blockchain acts as a timestamping service, we can choose to either use the block height or the block timestamp (UNIX timestamps). The Ethereum blockchain enables smart contract to track time by using $block.timestamp$. Miners do not accept blocks whose timestamp is more than 900 seconds after the previous one~\cite{blockvalidationalgorithm}. Because $MAX\_TIMEOUT$ is chosen to be significantly larger than the block time of Ethereum, it is economically not feasible to alter the time-stamping mechanism.

% %The reason we need a blockchain is twofold: first, we need to be able to order events without third-party (in order to know who acted in which order, since our protocol is purely sequential) and second, our protocol benefits from the permissionlessness of the blockchain, which means that any actor who can generate a public/private key pair is allowed to participate in the network. An additional constraint is that participants own some tokens of the underlying blockchain network we make use, called Ether in the case of Ethereum and Bitcoin in the case of Bitcoin.
% %A transaction must achieve eventual finality and be non-repudiable, non-malleable and permissionless (note that it still requires owning some tokens of the network)

% We assume that the buyer $B$ and the seller $S$ are capable of communicating over a non-blockchain based channel. This channel is not required to be secure and will solely be used for the purpose of negotiating the terms of the contract.

% Note that \name{}, in its original form, does not support the resumption of a previously failed protocol execution. We leave the extension for future work.

% Note that as transactions on the blockchain have a cost, it must hold that the total transaction costs are much lower than the value put into the smart contract, i.e.\ $F_p + D_B + D_S$  (cf. Section~\ref{sec:evaluation}).

\subsection{Threat Model}
Similar to Franklin et al.~\cite{franklin1997fair}, we consider \name{} fair if the file exchanged is consistent with the known hash value. Further formalizing on the attacker model in Section~\ref{sec:attackermodels}, we moreover define utility functions in Section~\ref{sec:utilityfunctions} to measure how $S$ and $B$ value $F$ along with the transmission of the file chunks. Under our rational adversary assumption, in any situation, a player takes action to maximize the final economic benefits. An adversary is not willing to perform an attack if the financial return is lower than the payoffs of following the protocol (i.e.\ $F_p + D_S$ for $S$ and $D_B + F_v$ for $B$). We also assume the trade only proceeds s.t.\ $F_c\leq F_p$ and $F_p\leq F_v$.

\subsection{Attack Analysis}\label{sec:attackanalysis}
\label{attack_analysis}
{\color{blue}
In this section, we analyze considered malicious behaviours.
\paragraph{\textbf{$S$ doesn't have any knowledge of $F$ and trades with $B$}} Our mechanism guarantees that $S$ loses the deposit performing this attack while with no financial incentive. Selling an unpossessed file is thus an irrational attack.

\paragraph{\textbf{$S$ sends chunks out of order}} In each round, $B$ only expects the chunk with the target hash value and considers others invalid, even though $S$ sends a chunk belongs to $F$. Sending chunks out of order is deemed to be malicious.

\paragraph{\textbf{$S$ sends all chunks but $c_1$ for an encrypted file}} This attack results in that $B$ receives a useless file. The payoff for $S$, in case $B$ reports and then $S$ proves, is $\frac{n-1}{n}\cdot F_p + F_c$, whereas the honest payoff for $S$ is $F_p + D_S$. Therefore, this attack is ruled out by choosing the seller's deposit, s.t.\ $D_S > F_c - \frac{1}{n} \cdot F_p$.

\paragraph{\textbf{$S$ does not send any file chunk $c_k$ or sends a wrong chunk, and $B$ may be forced to acknowledge it in fear of losing deposit $D_B$}} The possibility for $B$ to acknowledge a undelivered chunk gives $S$ an incentive not to send some chunk, because $B$ will acknowledge it anyway to get the deposit back. We introduce a counter-intuitive mechanism of offering $S$ the option to report that $B$ acknowledged some chunk $c_k$ without receiving it. If $B$ on the next step fails to prove, then $S$ receives the whole sum $D_S + D_B + F_p$ . Therefore, the buyer will never acknowledge a undelivered chunk.

\paragraph{\textbf{$B$ extorts $X$ from $S$ after the protocol initiated. Otherwise, the buyer will report dishonesty of the seller}} If disagreeing, $S$ will lose the deposit $D_S$ and receives $F_p/n$. Otherwise, $S$ can recover $D_S+F_p-X$ until the protocol is finalized successfully. This attack seems practical when $X < D_S+\frac{n-1}{n}\cdot F_p$. However, the optimal strategy of $B$ is to blackmail $S$ in the next every round till the end, which means $S$ will lose more if surrendering. Therefore, the best response of $S$ is to revolt rather than to surrender. Given that both $S$ and $B$ are rational and $B$ knows $S$ is rational, $S$ will not initiate this extortion attack because $S$ is not going to agree.

\paragraph{\textbf{$B$ does not acknowledge $c_2$, report not receiving $c_2$ and try to brute-force search $c_1$ if $c_1$ is low-entropy}} The buyer may crack the last chunk successfully, but, once the seller prove with $M^2_{CL}$, the buyer will recover $\frac{2}{n}\cdot F_p$ but lose the deposit $D_B$. So this attack is irrational with a reasonably large $D_B$. Similarly, the attack that $B$ doesn't acknowledge $c_1$ doesn't apply due to the risk of losing deposits.
}

\subsection{Utility functions}
\label{sec:utilityfunctions}
Files differ on how the seller and the buyer value them, in particular regarding individual file chunks. This is relevant for calculating optimal deposit sizes for the existence of a subgame perfect Nash Equilibrium. In practice, though, we do not necessarily know how each participant values a particular file; we, therefore, analyze the worst possible case and find participants' deposits in such a way that the honest behavior is always the subgame perfect Nash Equilibrium.
We use a special deposit refunding scheme to achieve that the honest behavior of both seller and the buyer is the subgame-perfect equilibrium solution, see \cite{gersbach} for related schemes. 


For some files, the utility function of a participant may grow close to linear (e.g.\ image files\footnote{We acknowledge that image files might be compressed in such a way that coarse-grained details are first transmitted.}, movies), while other files are only valuable in their entirety (e.g.\ encrypted/compressed files). The third category of files might be files where the value of the first chunk outweighs the value of the sum of all other chunks heavily.

We define $g^x(k)$ to be the relative utility function, for party $x \in \{Buyer, Seller\}$, after $k$ chunks of the file $F$ are sent. Note that the utility function of the buyer, $g^B(k)$, is monotonically increasing with the number of chunks as he gains more information about the file; on the other hand the utility function of the seller, $g^S(k)$, is monotonically decreasing with the number of chunks as he loses exclusivity of the file.
In order to prove that our protocol is incentive-compatible (it is in the participants' best interest to follow the rules), we analyze the arbitrary utility functions of the buyer and the seller in a rational adversary setting.


\subsubsection{Require the entire file}
For encrypted files, the utility function of the buyer is 0 until the chunk $c_1$ is received (cf. Equation~\ref{eq:entirefile1}).
\begin{equation}\label{eq:entirefile1}
  g^{B}(k) = \left\{
    \begin{array}{@{}l@{\thinspace}l}
       1 \text{, if } k=n \\
       0 \text{, otherwise} \\
    \end{array}
   \right.
\end{equation}

The worst case for the buyer is that the seller's utility function is as follows (cf. Equation~\ref{eq:entirefile2}).
\begin{equation}\label{eq:entirefile2}
  g^{S}(k) = \left\{
    \begin{array}{@{}l@{\thinspace}l}
       0 \text{, if } k=n \\
       1 \text{, otherwise} \\
     \end{array}
   \right.
\end{equation}

In that case, the seller wants the exact opposite of the buyer: he wants to send all the chunks except the last one, while the buyer is only interested in the last chunk.
\name{} therefore requires the deposit of the seller to be sufficiently high, to guarantee that the seller will send the entirety of the file.

\subsubsection{Only require the first chunk}
Recall, that the first chunk that the seller sends corresponds to the end of the file (containing padding and the file length). In some cases, the buyer may solely be interested in knowing this first chunk, for example if he only needs to know the length of the file or in some specific situations where the last chunk is particularly valuable (cf. Equation~\ref{eq:firstchunk1}).
\begin{equation}\label{eq:firstchunk1}
  g^{B}(k) = \left\{
    \begin{array}{@{}l@{\thinspace}l}
       1 \text{, if } k \geq 1 \\
       0 \text{, if k = 0} \\
     \end{array}
   \right.
\end{equation}


The worst case for the seller would be that the buyer's utility function is the exact opposite of the seller (cf. Equation~\ref{eq:firstchunk2}), because after receiving just the first chunk, the buyer already has no incentive to continue the transfer. Yet, the smart contract will only reward the seller with $\frac{1}{n} \cdot F_p$. From the perspective of the buyer, the bulk of the value has already been exchanged (that is, the buyer has already received a value of $F_v$, although the seller only received $\frac{1}{n} \cdot F_p$).
\begin{equation}\label{eq:firstchunk2}
  g^{S}(k) = \left\{
    \begin{array}{@{}l@{\thinspace}l}
       0 \text{, if } k \geq 1 \\
       1 \text{, if k = 0} \\
     \end{array}
   \right.
\end{equation}

All the remaining possible utility functions lie in between these two extremes. In the following section, we make use of the observations derived from the behavior of our mechanism to parametrize the buyer's and seller's deposits, $D_B$ and $D_S$, in such a way that honest behavior is a Nash Equilibrium. This implies that it is in both participants' best interest to behave honestly, as the deposits they provide to the smart contract are high enough and the deposit refunding scheme guarantees higher utility in case of honest behavior than in case of misbehaving.

\subsection{Subgame perfect Equilibrium}\label{sec:nashequilibrium}

In this section, we show that honest behavior in \name{} is a subgame perfect Nash equilibrium.

\subsubsection{Preliminaries}

 We denote the game with $G$. There are two players in $G$, seller and buyer. Game $G$ is sequential, players take their decisions one after another. The strategies available to the seller depending on the level of the game are the following: sending the file chunk, not sending the file chunk, prove sending the file chunk, timing out, reporting the wrong acknowledgment of the buyer and not reporting the wrong acknowledgment. The strategies available to the buyer are acknowledgment of the receipt of the file chunk, claiming not receiving the file chunk, timing out and proving the receipt of the file chunk.  

In order to guarantee honest behavior from both participants, mechanism require them to deposit a monetary amount, $D_B$ for the buyer and $D_S$ for the seller. The \name{} protocol sets what those deposits should be, depending on the price $F_p$ agreed upon. Recall that the smart contract has authority over the money sent by the participants; in case of misbehavior, the smart contract acts as an impartial judge for dispute mediation and distributes payoffs according to the protocol as specified in Table~\ref{tab:payouts}.

\subsubsection{Double Auction}
Note that exchanging the file and setting price is an instance of the double auction problem~\cite{myerson}. In the double auction, a single seller is the owner of one item which is traded with a single buyer. Both the seller and the buyer have privately known values for consuming the item, in our case $F_c$ for the seller and $F_v$ for the buyer. These values are unknown to the mechanism. Intuitively, there are three minimal requirements for the "good" mechanism, individual rationality: the participation of the agents is voluntary, meaning that at any point they may leave the mechanism and consume their initial endowments. The second requirement is budget balance: the mechanism is not allowed to subsidize the agents or to make any profits, the latter means that the amount paid by the buyer is completely transferred to seller. The third requirement is incentive compatibility (IC), meaning that reporting true valuations is the best strategy for both seller and the buyer. 
The seminal paper of Myerson and Satterthwaite \cite{myerson} studies the double auction problem. The well-known impossibility result states that in this setting there is no
mechanism which is fully efficient and at the same time is incentive compatible, individually rational and budget balanced. Blumrosen and Dobzinski~\cite{blumrosen} design an approximately efficient mechanism for achieving optimal expected social welfare function,  that is equal to the maximum of the two private values $F_c$ and $F_v$. In other words, the optimal social outcome is achieved when the item goes to the person who values it the most. It is proved that the only mechanism which satisfies the three properties discussed above is a posted price auction, in which the mechanism posts some price, in our setting $F_p$, if $F_c\leq F_p$ and $F_p\leq F_v$ then the trade takes place. Buyer pays $F_p$ to the seller and gets the item. If one of the conditions does not hold, then no trade takes place. The posted price mechanism is clearly individually rational, because the utilities of both players are non-negative in either case. Reporting true values is clearly a dominant strategy for both players, because reports from both sides do not affect their payoffs, in the calculation of the utility only the private value is used. If any of the players changes the true anticipated outcome of the mechanism, it only decreases his utility. Blumrosen and Dobzinski \cite{blumrosen} design the mechanism which achieves a social welfare that is equal to 0.63 times the optimal social welfare, given only the probability distribution on the value $F_v$. On the negative side, Leonardi et al. \cite{leonardi} prove that there is no mechanism which approximates the optimum by more than a factor of $0.74$ in the worst case. Although, providing efficient posted price can also be integrated into our mechanism, at this point we assume that agreeing on the price $F_p$ is done outside \name{}. Over the time, information can be aggregated to refine probability distributions of the valuations and consequently, more efficient posted price mechanisms can be implemented. 

\subsubsection{Finding the right size for deposits}

In this section, we will determine the optimal sizes for the deposits of both players of the game, in order to guarantee that the honest behavior of both players corresponds to the subgame-perfect equilibrium solution. 

\begin{theorem}
\label{subgame_perfectness}
There exist deposits $D_S$ and $D_B$ such that honest behavior of both players corresponds to the subgame-perfect Nash equilibrium of the extensive form game $G$.
\end{theorem}
\begin{proof}
See Appendix~\ref{proof}.
\end{proof}

%Note that subgame perfect equilibrium solution is robust to the case where a (malicious) buyer may have a file already. 

From the analysis we exclude the case where a (malicious) buyer may have a file already. In this case, it is possible that a buyer acknowledges the receipt of the chunk he has not received, and the rationality analysis boils down to the belief of the seller about the state. Note that given the seller believes the buyer does not have a file, he will send each chunk anyway. Our analysis solves this case.  

It is easy to observe that the linear refunding scheme by the mechanism of the price $F_p$ is arbitrary and serves only the purpose of simplicity and fairness. 

Attacks in the form of blackmail do not work. This is guaranteed by the assumptions of rationality and complete knowledge. If any of the parties blackmails the other, asking to collaborate or, otherwise he will make the other party lose deposit, the other party can ignore this kind of threat. Since the other party knows the blackmailing party is rational, the threat will never be realized. 

One chunk of the file is displayed on blockchain, in case of dispute. This can, in principle, be exploited by malicious buyers, to reveal the file chunk by chunk. On the other hand, since for each chunk they will lose a complete deposit, this is not a rational way to behave. 

{\color{blue}
\subsection {Secure Multi-Party Exchange}
\label{sec:securemultipartyexchange}
As file segments are exchanged independently, multi-party exchanges are secure as long as all segments are exchanged securely. We prove in Appendix~\ref{proof} that honest behaviour corresponds to a subgame perfect Nash equilibrium in the single seller case when both $D_S$ and $D_B$ are at least $F_p$. Similarly, in the multi-party case, the security of a single thread relies on the conditions that \textbf{(1)} the buyer's deposit for a segment is not smaller than the segment price (i.e.\ $D_B/z \geq F_p/z$); \textbf{(2)} the selling cost of a segment is not larger than the seller's deposit for a segment.

We reasonably conclude that the files where value is evenly distributed (e.g.\ images and movies) meet both conditions if $D_S \geq F_p$ and $D_B \geq F_p$. However, for the value-concentrated files, the selling cost of a single segment varies from $0$ up to $F_p$. Therefore, $D_S$ is required to be increased to at least $z\cdot F_p$ in order to preserve the security properties in every exchanging thread.

% We regard the P2P exchange as multiple independent threads of single seller exchanges, each thread holds the same security properties. We prove in Appendix~\ref{proof} that honest behavior corresponds to a subgame perfect Nash equilibrium in a single thread, which implies that following the protocol in all threads is the optimal behavior for colluding sellers.
}

==> sections/6.Evaluation.tex <==
\section{Implementation and Evaluation}\label{sec:evaluation}
\name{} is a symbiosis of an off- and on-chain component: an Ethereum smart contract serves for dispute mediation; and, an off-chain client is responsible for the actual file transfer (note that the off-chain client needs to regularly check the smart contract state). We implement the off-chain component as a browser application written in Typescript ($7\,500$ LOC), while the Ethereum component is a Solidity smart contract ($728$ LOC). The most significant functions of the smart contract are described in Appendix~\ref{sec:appendiximplementation}.

The seller and buyer clients first establish a WebRTC connection. Once the connection is established, the protocol as described in Algorithm \ref{alg:protocol_pseudocode} is executed. Note that both clients are required to be synchronized with the blockchain.

{\color{blue}
In consideration of the weakness of SHA-1~\cite{stevens2017first}, we chose SHA-256 as the cryptographic compression function. We re-implemented the SHA-256 hash function on the smart contract and the clients, such that we can execute the Merkle-Damg\aa rd construction on individual file blocks. We also implemented a zkSNARK contract for the privacy-preserving possession verification.
}

\paragraph{\textbf{On-chain Costs}}
Given no dispute, the on-chain operations of starting a sale, purchasing a file, starting a dispute and finalizing an exchange, cost below $170\,000$ gas (\$$0.07$ at a gas price of $3$ GWei\footnote{At the time of writing, the US dollar to Ether exchange rate is around \$$150$/Ether.}). {\color{blue} In \name{}, the most expensive transaction is to resolve a dispute by verifying the possession of a block of 64 bytes. A cleartext verification by calculating SHA-256 hash directly costs about $350\,000$ gas (\$$0.16$), whereas the zkSNARK scheme costs $1\,658\,000$ gas (\$$0.75$)}.
The cost is constant regardless of the file size or chunk size. In a P2P setting, verifying a BLS signature costs approximately $365\,000$ gas (\$$0.16$)~\cite{kfichter69:online}. We estimate the cost of purchasing a file from $10$ sellers to be below $450\,000$ gas (\$$0.2$).

Assuming a PoW blockchain supports ten transactions per second, this amounts to $864\,000$ transactions per day. An estimated upper limit of \name's throughput is thus $432\,000$ P2P downloads per day. This holds assuming the absence of disputes and assuming that a seller is ``re-using'' its collateral for $F$. Note that the measured number of daily downloads via BitTorrent between Dec’03 to Jan’04, is in the range of $237\,500$ to $576\,500$~\cite{pouwelse2005bittorrent}.

{\color{blue}
\paragraph{\textbf{Off-chain Messages}}
Transmitting a file of $n$ chunk requires $n$ rounds of interactions between the seller and buyer. The chunk length can be adjusted flexibly without increasing any on-chain cost (e.g.\ a file of $256$MB tranmistted in chunks of $256$KB needs $1024$ rounds of interactions which would be reduced to $512$ if increase the chunk size to $512$KB). 
}

==> sections/7.RelatedWork.tex <==
\section{Related Work}\label{sec:relatedwork}
Fair exchange has been extensively studied regarding fair multiparty computation \cite{bentov2014use,andrychowicz2014fair,andrychowicz2014secure,banasik2016efficient,bao1999multi,kilincc2015optimally,lysyanskaya2006rationality}, fair multiparty exchange \cite{franklin1997fair,asokan1998optimistic,park2003constructing,dodis2003breaking,zhou2000some,kupccu2010usable,garay2003timed,brickell1987gradual}, contract signing \cite{ateniese1999efficient,gauthierdickey2014secure,bao1998efficient,boldyreva2003threshold} and proof of ownership \cite{halevi2011proofs,di2012boosting}, which we discuss further in Appendix~\ref{apx:relatedwork}.

In the following, we mainly discuss related solutions based on permissionless blockchains. NashX~\cite{nashx} uses the Bitcoin blockchain and Nash equilibria to trade goods with the help of a trusted third party. It is not resistant against extortion attacks, even against a rational adversary, is not automatic and does not provide integrity verification. Darkleaks by Juels et al.~\cite{juels2016ring} enable a seller to collect donations for leaking a secret. Darkleaks does not guarantee file integrity and requires to upload the hash of each segment to the smart contract on the blockchain, which is impractical for large files; for a typical file with $100\,000$ segments, the costs would be above \$$2\,400$. FairSwap by Dziembowski et al.~\cite{dziembowski2018fairswap} allows secure digital content exchange through sending ciphertexts off-chain and revealing the key on-chain. FairSwap relies on a judge smart contract to arbitrate the misbehavior of the sender. FairSwap has a variable cost of dispute mediation --- there is a trade-off between the cost and the amount of additional off-chain data, while the cost of \name is constant. Despite its provable security, FairSwap does not offer a punishment scheme, which means the trading parties will not suffer any economic loss for any dishonesty. Therefore, we consider FairSwap is weakly fair compared to \name.

% \begin{table*}[!htb]
% \centering
% \begin{tabular}{@{}lllll@{}}
% \toprule
% Properties &                Our &                       [4] & [1337] & [99] \\ \midrule
% Integrity verification &    Practical &                 yy &  &  \\
% Use of TTP &                Yes, decentralized &         &  &  \\
% Memory complexity &         $O(1)$ &                     &  &  \\ 
% Time complexity &           $O(L)$ &                     &  &  \\ 
% Number of messages &        5 &                          &  &  \\ 
% Native value transfers &    Yes &                        &  &  \\
% Permissionless &            Yes &                        &  &  \\
% Fairness &                  Yes* &                       &  &  \\
% Assumptions &               Rational adversary &         & & \\
% Overhead &                  <10\% &                      &  &  \\
% Practicality &              Sure thing yo &              &  &  \\ \bottomrule
% \end{tabular}
% \caption{Comparison of related work and their respective properties.}
% \label{tb:relatedwork}
% \end{table*}

% \begin{table*}[!htb]
% \centering
% \caption{Comparison of related work and their respective properties.\todo{TODO}}
% \begin{tabular}{@{}lllll@{}}
% \toprule
% Properties &  \name{} &   FairSwap\cite{dziembowski2018fairswap} \\ \midrule
% % Integrity verification &      &                 & \\
% %Memory complexity &         $O(1)$ &    $O(1)$             \\ 
% Number of off-chain messages &   $2\times\text{number of file chunks}$ &    1  \\ 
% Number of on-chain transactions &   $3\sim 6$   &  $1\sim 2$    \\ 
% Dispute costs &     &     & \\
% Fairness &      strong       &       weak           \\ \bottomrule
% \end{tabular}
% \caption{123}
% \label{tb:relatedwork}
% \end{table*}


%\textbf{Complete Hiding of the File in Case of Disputes:} 
%Because the Ethereum's ledger is public, any transaction made on the network is visible to every node in the network. In the case of dispute, the mediation mechanism of \name{} requires the seller to send the concerned chunk $k$, which may contain valuable data. In the following we discuss possible extensions that provide better privacy guarantees than the standard \name{} protocol.
%We believe that using a zk-snarks~\cite{ben2013snarks} enabled smart contract blockchain platform like Hawk~\cite{kosba2016hawk}, the smart contract could keep the entire file private even in case of disputes (while in our work, the seller has to reveal the disputed chunk, e.g., 64 bytes in SHA256).



%The seller and the buyer each choose a random nonce $Nonce_B$, respectively $Nonce_S$. The buyer sends $Nonce_B$ to the seller along with the challenge hash $Challenge_{Hash}$ (cf. Equation~\ref{eq:challenge}):
%\begin{equation}\label{eq:challenge}
%Challenge_{Hash} = H(H(F) || Nonce_B || Nonce_S)
%\end{equation}
%The seller searches through the list of files he owns to see if one matches the $Challenge_{Hash}$. If one does match, then he knows that the buyer wants this file.
%}

%The seller consequently sends his Ethereum address, $Pub_S$, to the buyer. The buyer then deploys the \name{} smart contract to the Ethereum network and specifies within the smart contract the seller address $Pub_S$. This effectively restricts the participation to $Pub_S$ for this particular smart contract.}

%which makes it only possible for this address (public key) to accept the contract.

%Note that even if the communication channel between the buyer and the seller is insecure, an adversary could at most change the file hash or the seller's address.
%If the adversary modifies the file hash, the buyer will create the contract for an invalid file. The adversary, however, cannot profit from this misbehavior 

%but no benefit can be obtained by the adversary, since he does not own the file. If he did own the file, it would be rational for him to simply execute the protocol as instructed.
%{\color{red}faux, the adversary can just provide a file whose hash matches the hash.}

%In the second case (he changes the address), then the buyer will also create the contract, but if the adversary does not own the private key related to the public key, he simply won't be able to enter the contract. Since the buyer can void the contract at any time *before* the seller entered it, the worst that can happen to the buyer is having created the contract for nothing.
%}

%\subsection{A decentralized Spotify/Netflix / finding peers with the file}

%Using our protocol, it is possible to enable peer-to-peer file transfers for any kind of digital content, like music and movies. Assuming the hashes of the digital assets are known, which could be done by using the Kademlia protocol and distributed hash tables (DHT), like it is done for torrent files; the difference would be that while people keep the hashes of many files, the transfers would only be done 1 to 1. The protocol could be based on a reputation system, where a participant would trust some participants more than others, and trust the friends of their friends more than strangers. This indirectly serves as an anti-spam system for digital assets, as more reputable files will get more exposure. Reputation could be backed by an Ethereum token that holds some value, in order to make gaming the system costly and therefore uninteresting. This uses similar principles as the reputation-backed prediction market Augur.
% {\color{blue}
% \section{Extensions}
% An important extension we consider is to apply \name{} on peer-to-peer file sharing (e.g. BitTorrent) where a buyer can purchase from multiple sellers and download concurrently. To realize this, files are split into segments, which are exchanged separately. Segments are exclusive parts of the file which are composed of adjacent file chunks. Contrary to one-to-one scheme where each file is identified by a hash value, multi-to-one transfer requires the bundle of all the segments' hashes as the identity so that the authenticity of every segment can be verified individually. Similar to the chunk hash, the segment hash is also defined as the intermediate hash of the last block inside the segment, which means there is no additional computing overhead for segment hashes.
% Figure \ref{fig:segment} illustrates a two-segment file where each segment consists of two two-block chunk. 

% }

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=0.45\textwidth]{figures/segment_chunk_block.pdf}
% \caption{}
% \label{fig:segment}
% \end{figure}

==> sections/8.Conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

In this work, we present a practical and efficient protocol, which allows a buyer to purchase a file from one or multiple sellers. The buyer is assumed to know the cryptographic hash of the file, which allows us to perform an automated dispute mediation through a blockchain based smart contract.
We show that honest behavior in \name{} is a Nash equilibrium under a rational adversary. Under honest execution of the protocol, our implementation only requires three on-chain transactions for the exchange of any file size. In the case of disputes, we require up to two additional on-chain transactions. Contrary to previous work, \name{} has an inherent integrity verification, for every exchanged file chunk. The value transfer between the seller and the buyer is exchanged seamlessly because we make use of the Ethereum blockchain. Finally, by implementing the \name{} smart contract component, we show that the protocol execution is practical.

%\begin{acks}
%\begin{itemize}
%    \item "Denis Milicevic <denis@oraclize.it> Thanks for contacting me. Yes, you may make use of the SHA1 implementation. I have also checked with Oraclize, (whom it was created for) and they are fine with it too with proper credits. You may accredit it to "Denis Milicevic, Software Engineer at Oraclize LTD". Good luck on the paper, and when you do publish it, I'd appreciate if you send a link if possible, as it seems like the subject matter may be of interest."
%    \item Gary Bécigneul
%    \item Salomon Faure
%    \item Ralf Sasse
%    \item Hubert Ritzdorf
%\end{itemize}
%\end{acks}

\clearpage

==> sections/Abstract.tex <==
\subsection*{Abstract}
Digital contents are typically sold online through centralized and custodian marketplaces, which requires the trading partners to trust a central entity. We present \name, a fair protocol which, assuming the cryptographic hash of the file of interest is known to the buyer, is trust-free and lets a buyer purchase data for a previously agreed monetary amount, while guaranteeing the integrity of the contents. To prevent misbehavior, \name guarantees that any deviation from the expected participants' behavior results in a negative financial payoff;  i.e.\ we show that honest behavior corresponds to a subgame perfect Nash equilibrium. Our novel deposit refunding scheme is resistant to extortion attacks under rational adversaries. If buyer and seller behave honestly, \name's execution requires only three on-chain transactions, while the actual data is exchanged off-chain in an efficient and privacy-preserving manner. We moreover show how \name enables a flexible peer-to-peer setting where multiple parties fairly sell a file to a buyer.
